RadarPillars: Efficient Object Detection from 4D Radar Point Clouds

Automotive radar systems have evolved to provide not only range, azimuth and Doppler velocity, but also elevation data. This additional dimension allows for the representation of 4D radar as a 3D point cloud. As a result, existing deep learning methods for 3D object detection, which were initially developed for LiDAR data, are often applied to these radar point clouds. However, this neglects the special characteristics of 4D radar data, such as the extreme sparsity and the optimal utilization of velocity information. To address these gaps in the state-of-the-art, we present RadarPillars, a pillar-based object detection network. By decomposing radial velocity data, introducing PillarAttention for efficient feature extraction, and studying layer scaling to accommodate radar sparsity, RadarPillars significantly outperform state-of-the-art detection results on the View-of-Delft dataset. Importantly, this comes at a significantly reduced parameter count, surpassing existing methods in terms of efficiency and enabling real-time performance on edge devices.

==> tables/combined_methods.tex <==
\begin{table}[h!]
  \caption{Ergebnisse für die Kombination der einzelnen Methoden.}
  \label{tab:combined_methods}
  \renewcommand{\arraystretch}{1.2}
  \centering
  \sffamily
  \begin{footnotesize}
  \resizebox{1\columnwidth}{!}{
    \begin{tabular}{lllll|llll|l}
    \toprule
     & \multicolumn{4}{c|}{Entire Area} & \multicolumn{4}{c|}{Driving Corridor} & \\
    
    Features & {$mAP$} & {\splitcell{Car}{$AP_{50}$}} & {\splitcell{Pedestrian}{$AP_{25}$}} & {\splitcell{Cyclist}{$AP_{25}$}} & {$mAP$} & {\splitcell{Car}{$AP_{50}$}} & {\splitcell{Pedestrian}{$AP_{25}$}} & {\splitcell{Cyclist}{$AP_{25}$}} & {\splitcell{Framerate}{$Hz$}} \\
    \midrule
    Baseline \cite{PointPillars} & 39.5 & 30.2 & 25.6 & 62.8 & 60.9 & 61.5 & 36.8 & 84.5 & 20.6 \\
    \hline
    +\(v_{abs,xy}\) & 43.3 & 37.4 & 29.6 & 62.9 & 65.9 & 70.6 & 40.9 & 86.0 & 19.8 \\
    +\(v_{abs,xy}\), BB-Scaling & 43.8 & 35.8 & 31.0 & 64.5 & 65.8 & 70.1 & 42.5 & 84.9 & 35.2 \\
    +\(v_{abs,xy}\), BB-Scaling, PA & 45.4 & 37.7 & 34.6 & 63.9 & 66.4 & 69.9 & 46.3 & 82.9 & 34.3 \\
    \bottomrule
    \end{tabular}
    }
  \end{footnotesize}
  \rmfamily
\end{table}


% \begin{table}[h!]
%   \caption{Ergebnisse für die Kombination der einzelnen Methoden.}
%   \label{tab:combined_methods}
%   \renewcommand{\arraystretch}{1.2}
%   \centering
%   \sffamily
%   \begin{footnotesize}
%   \resizebox{1\columnwidth}{!}{
%     \begin{tabular}{lllll|llll|l}
%     \toprule
%      & \multicolumn{4}{c|}{Entire Area} & \multicolumn{4}{c|}{Driving Corridor} & \\
    
%     Features & {\rotatebox[origin=l]{90}{mAP}} & {\rotatebox[origin=l]{90}{Car}} & {\rotatebox[origin=l]{90}{Pedestrian $AP_{50}$}} & {\rotatebox[origin=l]{90}{Cyclist}} & {\rotatebox[origin=l]{90}{mAP}} & {\rotatebox[origin=l]{90}{Car}} & {\rotatebox[origin=l]{90}{Pedestrian}} & {\rotatebox[origin=l]{90}{Cyclist}} & {\rotatebox[origin=l]{90}{Runtime}} \\
%     \midrule
%     Baseline & 39.5 & 30.2 & 25.6 & 62.8 & 60.9 & 61.5 & 36.8 & 84.5 & FILL \\
%     \hline
%     \(v_{abs,xy}\) & 43.3 & 37.4 & 29.6 & 62.9 & 65.9 & 70.6 & 40.9 & 86.0 & FILL \\
%     \(v_{abs,xy}\), BB-Scaling & 43.8 & 35.8 & 31.0 & 64.5 & 65.8 & 70.1 & 42.5 & 84.9 & FILL \\
%     \(v_{abs,xy}\), BB-Scaling, PA & 45.4 & 37.7 & 34.6 & 63.9 & 66.4 & 69.9 & 46.3 & 82.9 & FILL \\
%     \bottomrule
%     \end{tabular}
%     }
%   \end{footnotesize}
%   \rmfamily
% \end{table}

==> tables/eval_comparisons.tex <==
\begin{table}[h!]
  \caption{Ergebnisse der Implementierung verschiedener Backbones auf dem Validierungs-Split des View-of-Delft-Datensatzes.}
  \label{tabelle_effiziente_backbones_ergebnisse}
  \renewcommand{\arraystretch}{1.2}
  \centering
  \sffamily
  \begin{footnotesize}
    \resizebox{1\columnwidth}{!}{
    \begin{tabular}{lllll|llll}
    \toprule
     & \multicolumn{4}{c|}{Entire Area} & \multicolumn{4}{c}{Driving Corridor} \\
    
    Features & {\rotatebox[origin=l]{90}{mAP}} & {\rotatebox[origin=l]{90}{Car}} & {\rotatebox[origin=l]{90}{Pedestrian}} & {\rotatebox[origin=l]{90}{Cyclist}} & {\rotatebox[origin=l]{90}{mAP}} & {\rotatebox[origin=l]{90}{Car}} & {\rotatebox[origin=l]{90}{Pedestrian}} & {\rotatebox[origin=l]{90}{Cyclist}} \\
    \midrule
    Baseline & 39.5 & 30.2 & 25.6 & 62.8 & 60.9 & 61.5 & 36.8 & 84.5 \\
    \hline
    MobileNet & 38.0 & 31.5 & 24.3 & 58.3 & 60.9 & 67.2 & 33.9 & 81.5 \\
    MobileNetv2 & 38.6 & 32.1 & 26.0 & 57.7 & 62.2 & 67.8 & 35.4 & 83.3 \\
    YOLOv8-n & 38.3 & 29.4 & 27.6 & 57.8 & 61.4 & 64.3 & 38.9 & 81.0 \\
    YOLOv8-s & 39.6 & 30.1 & 30.3 & 58.3 & 63.7 & 66.1 & 41.1 & 83.8 \\
    \bottomrule
    \end{tabular}
    }
  \end{footnotesize}
  \rmfamily
\end{table}

==> tables/velo_1.tex <==
\begin{table}[h!]
  \caption{Ergebnisse der Untersuchung zum Einfluss der relativen und absoluten Radial-Geschwindigkeit auf dem Validierungs-Split des View-of-Delft-Datensatzes.}
  \label{tabelle_relabs_ergebnisse}
  \renewcommand{\arraystretch}{1.2}
  \centering
  \sffamily
  \begin{footnotesize}
  \resizebox{1\columnwidth}{!}{
    \begin{tabular}{lllll|llll}
    \toprule
     & \multicolumn{4}{c|}{Entire Area} & \multicolumn{4}{c}{Driving Corridor} \\
    
    Features & {\rotatebox[origin=l]{90}{mAP}} & {\rotatebox[origin=l]{90}{Car}} & {\rotatebox[origin=l]{90}{Pedestrian}} & {\rotatebox[origin=l]{90}{Cyclist}} & {\rotatebox[origin=l]{90}{mAP}} & {\rotatebox[origin=l]{90}{Car}} & {\rotatebox[origin=l]{90}{Pedestrian}} & {\rotatebox[origin=l]{90}{Cyclist}} \\
    \midrule
    PointPillars & 39.5 & 30.2 & 25.6 & 62.8 & 60.9 & 61.5 & 36.8 & 84.5 \\
    \hline
    PointPillars - \(v_{abs}\) & 32.3 & 33.7 & 20.1 & 43.2 & 58.6 & 70.8 & 29.6 & 75.4\\
    PointPillars - \(v_{rel}\) & 38.6 & 33.7 & 24.7 & 57.6 & 62.9 & 68.8 & 37.0 & 83.0 \\
    \bottomrule
    \end{tabular}
    }
  \end{footnotesize}
  \rmfamily
\end{table}

==> tables/velo_2.tex <==
\begin{table}[h!]
  \caption{Ergebnisse der Untersuchung des Einflusses vom Offsets der Punkte zu den mittleren Radial-Geschwindigkeiten auf dem Validierungs-Split des View-of-Delft-Datensatzes.}
  \label{tabelle_offset_relabs_ergebnisse}
  \renewcommand{\arraystretch}{1.2}
  \centering
  \sffamily
  \begin{footnotesize}
  \resizebox{1\columnwidth}{!}{
    \begin{tabular}{lllll|llll}
    \toprule
     & \multicolumn{4}{c|}{Entire Area} & \multicolumn{4}{c}{Driving Corridor} \\
    
    Features & {\rotatebox[origin=l]{90}{mAP}} & {\rotatebox[origin=l]{90}{Car}} & {\rotatebox[origin=l]{90}{Pedestrian}} & {\rotatebox[origin=l]{90}{Cyclist}} & {\rotatebox[origin=l]{90}{mAP}} & {\rotatebox[origin=l]{90}{Car}} & {\rotatebox[origin=l]{90}{Pedestrian}} & {\rotatebox[origin=l]{90}{Cyclist}} \\
    \midrule
    \textit{Baseline} & 39.5 & 30.2 & 25.6 & 62.8 & 60.9 & 61.5 & 36.8 & 84.5 \\
    \hline
    \textit{Baseline} + \(v_{rel,m}\) & 39.9 & 36.8 & 24.8 & 58.0 & 62.0 & 69.5 & 35.4 & 81.1  \\
    \textit{Baseline} + \(v_{abs,m}\) & 39.3 & 35.7 & 25.7 & 56.7 & 63.8 & 70.3 & 37.1 & 84.1 \\
    \textit{Baseline} + \(v_{rel,m},\ v_{abs,m}\) & 39.6 & 36.0 & 26.7 & 56.2 & 63.8 & 70.0 & 37.5 & 83.8 \\
    \bottomrule
    \end{tabular}
    }
  \end{footnotesize}
  \rmfamily
\end{table}

==> tables/velo_3.tex <==
\begin{table}[h!]
  \caption{Ergebnisse der Untersuchung des Einflusses der konstruierten x- und y-Komponenten der beiden Radial-Geschwindigkeiten als zusätzliche Features auf dem Validierungs-Split des View-of-Delft-Datensatzes.}
  \label{tabelle_relabsxy_ergebnisse}
  \renewcommand{\arraystretch}{1.2}
  \centering
  \sffamily
  \begin{footnotesize}
  \resizebox{1\columnwidth}{!}{
    \begin{tabular}{lllll|llll}
    \toprule
     & \multicolumn{4}{c|}{Entire Area} & \multicolumn{4}{c}{Driving Corridor} \\
    
    Features & {\rotatebox[origin=l]{90}{mAP}} & {\rotatebox[origin=l]{90}{Car}} & {\rotatebox[origin=l]{90}{Pedestrian}} & {\rotatebox[origin=l]{90}{Cyclist}} & {\rotatebox[origin=l]{90}{mAP}} & {\rotatebox[origin=l]{90}{Car}} & {\rotatebox[origin=l]{90}{Pedestrian}} & {\rotatebox[origin=l]{90}{Cyclist}} \\
    \midrule
    \textit{Baseline} & 39.5 & 30.2 & 25.6 & 62.8 & 60.9 & 61.5 & 36.8 & 84.5  \\
    \hline
    \textit{Baseline} + \(v_{rel,xy}\) & 41.8 & 37.9 & 26.0 & 61.4 & 64.2 & 69.4 & 37.8 & 85.4  \\
    \textit{Baseline} + \(v_{abs,xy}\) & 43.3 & 37.4 & 29.6 & 62.9 & 65.9 & 70.6 & 40.9 & 86.0  \\
    \textit{Baseline} + \(v_{rel,xy},\ v_{abs,xy}\) & 37.9 & 31.7 & 25.9 & 56.1 & 61.6 & 68.6 & 38.5 & 77.8  \\
    \bottomrule
    \end{tabular}
    }
  \end{footnotesize}
  \rmfamily
\end{table}

==> tables/velo_4.tex <==
\begin{table}[h!]
  \caption{Ergebnisse der Untersuchung des Einflusses des Offsets der Punkte zu den konstruierten x- und y-Komponenten der beiden Radial-Geschwindigkeiten als zusätzliche Features auf dem Validierungs-Split des View-of-Delft-Datensatzes.}
  \label{tabelle_offset_relabsxy_ergebnisse}
  \renewcommand{\arraystretch}{1.2}
  \centering
  \sffamily
  \begin{footnotesize}
  \resizebox{1\columnwidth}{!}{
    \begin{tabular}{lllll|llll}
    \toprule
     & \multicolumn{4}{c|}{Entire Area} & \multicolumn{4}{c}{Driving Corridor} \\
    
    Features & {\rotatebox[origin=l]{90}{mAP}} & {\rotatebox[origin=l]{90}{Car}} & {\rotatebox[origin=l]{90}{Pedestrian}} & {\rotatebox[origin=l]{90}{Cyclist}} & {\rotatebox[origin=l]{90}{mAP}} & {\rotatebox[origin=l]{90}{Car}} & {\rotatebox[origin=l]{90}{Pedestrian}} & {\rotatebox[origin=l]{90}{Cyclist}} \\
    \midrule
    Baseline & 39.5 & 30.2 & 25.6 & 62.8 & 60.9 & 61.5 & 36.8 & 84.5  \\
    \hline
    \textit{Baseline} + \(v_{rel,xy,m}\) & 38.4 & 31.6 & 26.5 & 57.1 & 61.4 & 66.9 & 36.9 & 80.3  \\
    \textit{Baseline} + \(v_{abs,xy,m}\) & 39.9 & 31.2 & 28.9 & 59.6 & 62.0 & 65.2 & 39.1 & 81.8 \\
    \textit{Baseline} + \(v_{rel,xy,m},\ v_{abs,xy,m}\) & 38.6 & 33.1 & 26.7 & 56.0 & 64.3 & 69.7 & 39.2 & 84.0 \\
    \bottomrule
    \end{tabular}
    }
  \end{footnotesize}
  \rmfamily
\end{table}
